Revisiting Perceptron: Efficient and Label-Optimal Learning of Halfspaces

It has been a long-standing problem to efficiently learn a halfspace using as few labels as possible in the presence of noise. In this work, we propose an efficient Perceptron-based algorithm for actively learning homogeneous halfspaces under the uniform distribution over the unit sphere. Under the bounded noise condition~\cite{MN06}, where each label is flipped with probability at most $\eta < \frac 1 2$, our algorithm achieves a near-optimal label complexity of $\tilde{O}\left(\frac{d}{(1-2\eta)^2}\ln\frac{1}{\epsilon}\right)$ in time $\tilde{O}\left(\frac{d^2}{\epsilon(1-2\eta)^3}\right)$. Under the adversarial noise condition~\cite{ABL14, KLS09, KKMS08}, where at most a $\tilde \Omega(\epsilon)$ fraction of labels can be flipped, our algorithm achieves a near-optimal label complexity of $\tilde{O}\left(d\ln\frac{1}{\epsilon}\right)$ in time $\tilde{O}\left(\frac{d^2}{\epsilon}\right)$. Furthermore, we show that our active learning algorithm can be converted to an efficient passive learning algorithm that has near-optimal sample complexities with respect to $\epsilon$ and $d$.

==> discussion.tex <==
\section{Discussion and Open Problems}
In this work, we propose a perceptron-based algorithm for efficient active learning of homogeneous linear separators under uniform distribution with noise. Under both bounded noise condition and adversarial noise condition, our algorithm achieves near-optimal label complexity. Our results significantly improves over the existing results in \cite{ABL14, ABHZ16}.
%$\tilde{O}\left(\frac{d}{(1-2\eta)^2}\right)$

Our analysis is performed under uniform unlabeled data distribution. However, it can be easily generalized to any spherical symmetrical distributions, for example, isotropic Gaussian distributions. It can also be generalized to distributions whose densities with respect to uniform distribution are bounded away from 0.

There are still many open problems in learning linear separators efficiently with respect to both time and label requirements:

\begin{enumerate}
  \item Can perceptron-based algorithms, or other computationally efficient algorithms, be adapted to learn linear separator in the noisy setting, under more general data distributions (e.g. log-concave distributions) with optimal label complexity?
  \item Are there any computationally efficient algorithms that can learn under weaker noise conditions, for example, Tsybakov noise condition~\citep{T04}?
  \item Can we design efficient and label-optimal active learning algorithms without the knowledge of noise parameters?
  \item Our algorithm is based on perceptron, a classical algorithm for online learning. Can one design other active learning algorithms through the lens of online learning? A representative example is~\citet{H07b}, where the algorithm simulates equivalence queries using label queries.
  %, via the notion of {\em minimum specifiying sets}.
  Another interesting open question is, can one design a winnow-based algorithm~\citep{L87} for attribute and computationally efficient active learning?
\end{enumerate}
  %relation SGD
  %ptas using perceptron

